The KL3M Data Project: Copyright-Clean Training Resources for Large Language Models

Practically all large language models have been pre-trained on data that is subject to global uncertainty related to copyright infringement and breach of contract. This creates potential risk for users and developers due to this uncertain legal status. The KL3M Data Project directly confronts this critical issue by introducing the largest comprehensive training data pipeline that minimizes risks related to copyright or breach of contract. The foundation of this project is a corpus of over 132 million documents and trillions of tokens spanning 16 different sources that have been verified to meet the strict copyright and licensing protocol detailed herein. We are releasing the entire pipeline, including 1) the source code to acquire and process these documents, 2) the original document formats with associated provenance and metadata, 3) extracted content in a standardized format, 4) pre-tokenized representations of the documents, and 5) various mid- and post-train resources such as question-answer, summarization, conversion, drafting, classification, prediction, and conversational data. All of these resources are freely available to the public on S3, Hugging Face, and GitHub under CC-BY terms. We are committed to continuing this project in furtherance of a more ethical, legal, and sustainable approach to the development and use of AI models.

==> tables/token_statistics.tex <==
\begin{table}[htbp]
\centering
\caption{KL3M Dataset Token Statistics}
\label{tab:token_statistics}
\begin{tabular}{lrrrrr}
\toprule
Dataset & Documents & Total Tokens & Min & Mean & Max \\
\midrule
Court Listener (CAP) & 6,914,364.0 & 16,662,877,079.0 & 7 & 2,409 & 725,988 \\
Court Dockets & 641,942.0 & 7,358,649,911.0 & 526 & 11,463 & 14,094,071 \\
.gov Websites & 2,368,347.0 & 16,531,103,948.0 & 1 & 6,980 & 7,460,915 \\
Electronic CFR & 206,781.0 & 109,846,126.0 & 5 & 531 & 1,303,458 \\
SEC EDGAR Filings & 11,482,351.0 & 250,153,684,922.0 & 1 & 21,785 & 3,510,994 \\
EDGAR Agreements & 1,473,797.0 & 21,962,695,999.0 & 1 & 14,902 & 86,878,995 \\
EU Official Journal & 692,087.0 & 27,763,080,136.0 & 2 & 40,115 & 2,776,849 \\
Federal Depository Library & 279,093.0 & 7,441,183,130.0 & 2 & 26,662 & 7,272,240 \\
Federal Register & 3,115,383.0 & 13,545,126,193.0 & 4 & 4,347 & 2,519,508 \\
GovInfo & 7,382,699.0 & 57,732,359,438.0 & 1 & 7,819 & 10,631,622 \\
RECAP & 14,265,799.0 & 65,309,277,086.0 & 1 & 4,578 & 3,808,848 \\
RECAP Documents & 1,621,886.0 & 5,700,833,738.0 & 1 & 3,514 & 499,063 \\
Regulations.gov & 829,451.0 & 7,178,510,379.0 & 1 & 8,654 & 3,523,621 \\
UK Legislation & 74,709.0 & 730,990,628.0 & 43 & 9,784 & 1,409,059 \\
US Code & 68,759.0 & 69,638,458.0 & 2 & 1,012 & 182,974 \\
USPTO Patents & 6,413,827.0 & 81,575,351,620.0 & 87 & 12,718 & 3,469,801 \\
\midrule
Total & 57,831,275.0 & 579,825,208,791.0 & 1 & 10,026 & 86,878,995 \\
\bottomrule
\end{tabular}
\end{table}

